New Metrics to Evaluate the Performance and Fairness of Personalized Federated Learning

In Federated Learning (FL), the clients learn a single global model (FedAvg) through a central aggregator. In this setting, the non-IID distribution of the data across clients restricts the global FL model from delivering good performance on the local data of each client. Personalized FL aims to address this problem by finding a personalized model for each client. Recent works widely report the average personalized model accuracy on a particular data split of a dataset to evaluate the effectiveness of their methods. However, considering the multitude of personalization approaches proposed, it is critical to study the per-user personalized accuracy and the accuracy improvements among users with an equitable notion of fairness. To address these issues, we present a set of performance and fairness metrics intending to assess the quality of personalized FL methods. We apply these metrics to four recently proposed personalized FL methods, PersFL, FedPer, pFedMe, and Per-FedAvg, on three different data splits of the CIFAR-10 dataset. Our evaluations show that the personalized model with the highest average accuracy across users may not necessarily be the fairest. Our code is available at https://tinyurl.com/1hp9ywfa for public use.

==> Sections/system.tex <==
\section{Evaluation Framework for Personalization}
\label{sec:system}

% System Figure
% \begin{figure}[t!]
% \begin{center}
% \centerline{\includegraphics[width=1\columnwidth]{images/EvalFramework.pdf}}
% \caption{System Architecture}
% \label{fig:sysArch}
% \end{center}
% \end{figure}

\berkay{Because we are submitting a ML conference, I think we do not need to have a system like description. Additionally this will help page limitation of 6 pages. Here is my suggestion:
(1) Section 4 can directly introduce the Evaluation Metrics. This means that we can have Section 4.3 as Section 4. 

(2) We can move the (a) Dataset, (b) Dataset splitting strategies, (c) federated model generation and (d) Framework Implementation under "Evaluation Setup subsection" in Evaluation (we be sure that they are concise but provides necessary information to understand the experimental results.)

(3) We can comment out systems figure.

(4) In this way, I believe that paper flow will be better.
}

%In this section, we explain the system in more detail. 
%
Initially, the system selects the dataset and divides it according to the chosen data-split strategy among the chosen number of clients (Section~\ref{subsec:dataGenerator}).
%
The system then trains the \texttt{FedAvg} model and the other personalization algorithm-based models with the chosen model architecture (Section~\ref{sec:federatedModelGeneration}).
%
Finally, the performance of the trained models from the previous step are evaluated on a defined set of metrics (Section~\ref{sec:evaluationMetrics}). 
%
These metrics are divided into the following two groups: a \textit{performance} perspective (Section~\ref{subsec:performance_metrics}) and a \textit{fairness} perspective (Section~\ref{subsec:fairness_metrics}).

% Module 1.
\subsection{Data Generator}
\label{subsec:dataGenerator}
The \texttt{Data Generator} module is responsible for two tasks: ($1$) selecting the dataset to be used based on the user's choice and then ($2$) subsequently generating a data-split on this dataset, also based on the user's choice. The user also provides the number of clients to simulate, and after this process, the data is now split to mimic the \texttt{FL} setting. 
%We describe the datasets we support in Section~\ref{datasets_supported}, and the data-splits supported in Section~\ref{datasplits_supported}.
 
% Sub-subsection.
\shortsectionBf{Datasets.}
%\label{datasets_supported}
We currently support the CIFAR-10 and MNIST datasets, widely used in \texttt{FL} training in the literature.
%Still, it is straightforward to use other datasets.
%
MNIST is a dataset of $\mathtt{28 \times 28}$ images of handwritten digits from $\mathtt{0}$-$\mathtt{9}$ consisting of $\mathtt{10}$ labels and $\mathtt{70,000}$ instances. CIFAR-10 is a dataset of $\mathtt{32 \times 32}$ color images with $\mathtt{10}$ classes and $\mathtt{60,000}$ instances. 
%
Other well-known datasets such as CIFAR-100 and Imagenet, and custom datasets can be easily integrated to the framework.

%\berkay{what about model architectures?}
%\sid{Will include it under Federated Model Generation section. Also we won't be able to explain the architectures in detail, so I'll just cite the relevant paper which use those architecture(s).}

% Sub-subsection.
\shortsectionBf{Data-splitting Strategies.}
%\label{datasplits_supported}
The data splitting module supports the following four different data-splitting techniques.
%from the literature, detailed as follows. We plan to support other data-splits as well in the future.

In data-split 1 (\textbf{DS-1}), each user has the same total number of samples but may have different classes and a different number of samples per class.
%
The statistical heterogeneity is varied by controlling the parameter $\mathtt{k}$, which controls the number of overlapping classes between each user. 
%
For example, $\mathtt{k=4}$ corresponds to a highly non-identical data partition, whereas $\mathtt{k=10}$ corresponds to a highly identical data partition across the participating users. In our experiments, we set $\mathtt{k}$ to 4 to have non-IID data across users. 

%
In \textbf{DS-2}, all users have samples from all classes, but the number of samples per class they have is different, and hence the total number of samples per user is also different across users. 
%
%(Independent \& Identically Distributed)
In order to simulate a non-IID distribution, we assign samples from each class to the users using a Dirichlet distribution with $\mathtt{\alpha = 0.9}$, following the previous work~\cite{nIID_dist}. Each class is parameterized by a vector $\mathtt{q}$ where $\mathtt{q \geq 0, i \in [1, N]}$, where $\mathtt{q}$ is sampled from a Dirichlet distribution with parameters $\mathtt{\alpha}$ and $\mathtt{p}$. 
%
The parameter $\mathtt{p}$ is the prior class distribution over the classes, and $\mathtt{\alpha}$ is the concentration parameter that controls the data similarity among the users. 
%
If $\mathtt{\alpha \rightarrow \infty}$, all users have an identical distribution to the prior. If $\mathtt{\alpha \rightarrow 0}$, each user only has samples from one class randomly chosen. 

For \textbf{DS-3}, each user has two of the ten class-labels. 
%
Additionally, the total number of samples per user is different, \ie all the users do not have the same number of total samples. 
%
The samples assigned to users are drawn from a log-normal distribution with the parameters $\mathtt{\mu = 0}$ and $\mathtt{\sigma = 2}$.
%
A variable $\mathtt{u}$ has a log-normal distribution if $\mathtt{log(u)}$ is normally distributed. 
%
The probability density function for the log-normal distribution is computed as:

\begin{equation}
    \mathtt{p(u) = \frac{1}{\sigma u \sqrt{(2\pi)}} e^{-(\frac{(ln(u) - \mu)^2}{2\sigma^{2}})}}
    \label{eqn:eqn_2}    
\end{equation}

These parameters correspond to the underlying normal distribution from which we draw the samples.

% Describe the sampling process for DS-4.
\textbf{DS-4} is introduced in \texttt{Per-FedAvg}~\cite{metaFL_2}. In this technique, assuming there are $\mathtt{n}$ users, then the data is split as follows. Half of the users ($\mathtt{\frac{n}{2}}$), have $\mathtt{k}$ images of each of the first five classes, and the remaining users ($\mathtt{\frac{n}{2}}$), have $\mathtt{\frac{k}{2}}$ images from only \textit{one} of the first five classes and $\mathtt{2k}$ images from only \textit{one} of the remaining five classes. The parameter $\mathtt{k}$ is set as $\mathtt{k = 196}$ and $\mathtt{k = 68}$ for MNIST, and CIFAR-10 respectively.


\subsection{Federated Model Generation}
\label{sec:federatedModelGeneration}
In this module, the \texttt{FedAvg} model and the personalized \texttt{FL} algorithms supported (Section~\ref{subsec:implementation}) are trained, and their inferences on the test set are obtained for evaluation and comparison. 

\shortsectionBf{Model Architectures.}
Currently, we support the following model architectures commonly used in the literature. 
%
For the CIFAR-10 dataset, we use a CNN-based model with two 2-D convolutional layers separated by a MaxPool layer between them and followed by three fully connected (FC) layers.  
%
The fully connected layers have $400$, $120$, and $84$ hidden neurons. We use ReLu activations after each layer except the last FC layer.
%
For the MNIST dataset, we use a two-layer deep neural network (DNN) with $100$ hidden-layer neurons, with a ReLu activation on the hidden layer. 
%
The output layer has $10$ nodes with a softmax function to get the class probabilities. The architectures we use for both datasets are similar to those in \texttt{pFedMe} for conformity.
% 
Extensions to support other architectures is straightforward.

%\berkay{Please read one more time below very very carefully, line by line, and let me know. This is the key section. I will then review it.}
%\sid{Addressed. Made a couple passes.}

\subsection{Framework Implementation}
\label{subsec:implementation}
The \texttt{Data Generator} module of our framework currently supports two datasets (CIFAR-10 and MNIST), and four data-splits (\textbf{DS-1}, \textbf{DS-2}, \textbf{DS-3}, and \textbf{DS-4}).
%
In the \texttt{Evaluation Metrics} module, we implemented the metrics from a \texttt{performance} perspective (Section~\ref{subsec:performance_metrics}) and a \texttt{fairness} perspective (Section~\ref{subsec:fairness_metrics}).
%
We integrated the following \texttt{FL} algorithms into our framework: \sys, \sysGD, \texttt{FedPer}, \texttt{pFedMe}, and \texttt{Per-FedAvg}. 
%
We are limited by the non-availability of the code and the hyper-parameter details to replicate the other personalization algorithms' reported results. Thus, we have not included them in the current work.  
%
Our framework is implemented on Python $\mathtt{3.7}$, and a PyTorch version of $\mathtt{v1.3.1}$ and runs on an NVIDIA Tesla T4 GPU with $\mathtt{16GB}$ memory with a CUDA version of $10.0$ and a driver version of $410.104$. 


% In the \texttt{Federated Model Generation} module, we currently support the following personalization algorithms: \texttt{FedPer}, \texttt{Per-FedAvg}, \texttt{pFedMe}, \texttt{\sys}, and \texttt{\sysGD}.
%


==> backup/Version_1/BerkayNotes.tex <==
%https://docs.google.com/document/d/1fA6-V5dHB5KIRgDJMiQe0_wvaSr7f4kJ-nba8Gy394U/edit

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Conferences that we can submit:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

- ACM FAccT 2021 Call for Papers (Closed) Deadline 7 October 2020 Passed

- ECML PKDD is doable and there's a little over a month for the submission deadline.

- ICDM is also a good Data Mining Conference and has a longer period until the deadline.

- ICML-A (submission deadlines):
    +   Main Conference: July 3, 2021
    +   Special Sessions/Workshops/Challenges: August 6, 2021
    +   Notification of Acceptance: September 4, 2021
    
- Anything  interesting?

%%%%%%
Example papers for Framework (Please add any other sample libraries and papers)
%%%%%%

1- https://github.com/kleincup/DEEPSEC
https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=8835375

2- https://github.com/IBM/federated-learning-lib
https://arxiv.org/pdf/2007.10987.pdf --> MUST READ.

3- Evaluation Framework for Large-scale Federated Learning
https://arxiv.org/abs/2003.01575

%%%%%%
0- Introduction
%%%%%%%

%%%%%
Background:
%%%%%
What is Federated Learning -1-2 paragraphs
    -Give some details here, if possible introduce with a Figure
What is Personalization: 1-2 paragraphs, if possible include a Figure for personalization.

%%%%%%
Related Work [DONE]
%%%%%%
// KDD paper related work is very short--your thesis should have comprehensive related work. This will be helpful for your thesis's related work.

1- Start with a comprehensive related work, by comprehensive I mean more comprehensive than the KDD paper. Group the papers in different categories and introduce papers in each category.
- 
This is similar to the related work of the Adaptive Personalized Federated Learning paper.
You can use the similar categorization they have. In addition, check other personalization papers to see if you are missing anything, such as a category that does not exist in the Adaptive Personalized Federated Learning paper and come up with a global related work that is comprehensive and concise.

%%%%%%
Section: Problem Statement: [WORKING]
%%%%%%
Based on your study of these related works. List the problem you see, like this:

Problem 1- Diverse DataSplit Selection: Introduce the problem, and explain what this problem causes in the results.

Problem 2- Lack of Reporting Complete Results. Introduce the problem, and explain what this problem causes in the results.

Problem 3- Fairness Notion among Users.Introduce the problem, and explain what this problem causes in the results.

Problem 4- Model Architecture: Introduce the problem, and explain what this problem causes in the results.

Problem 5- ....: Introduce the problem, and explain what this problem causes in the results
...
...

%%%%%%
System
%%%%%%
1- Introduce the system with a Figure, explain each component briefly. [WORKING]
Then introduce each component in detail:

1.1 Datasets: Which datasets you support? Syntetic and Real datasets, why these datasets?
1- 2 paragraph. Check other personalization paper dataset sections and have a common one here that captures all the details they mention.

1.2 Data-Splitting Module [DONE]

1.3. ...

1.4. Evaluation Metrics [Novelty] [DONE]
    Categorize and Introduce each evaluation metric precisely, introduce formula and introduce why you have this evaluation metric.
    
1.5 Visualization -- Say we use X to support visualization of these metrics across datasplits, datasets etc.

In this section you can mention how did you implement the system, Python, which libraries do you use. Command line options to run the algorithms.
such as: \$PerEval -dataset mnist -split ds1 -metrics all -peruser yes -vis true. 

%%%%%%
EVALUATION
%%%%%%
- Introduce the algorithms that will be evaluated by the system.
- Report metrics in the table: Interpret the results (a little bit details)
- Visualize: Give some insights








==> backup/Version_1/TODOs.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
TODOs: -Sid.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%
March 15th:
%%%%%%%%%%%%%%%%%%%%%%%%

* On how to improve the presentation of Table 2 (related works). Maybe use a map of numbers between numbers and the names of the datasets used? [Addressed.]

* On changing the names of the columns of Table 2? [Addressed for now.]

* On the addition of additional columns to Table 2?
    - Maybe also have a column where we check if the reported works report the number of communication rounds or not, if not mentioned then maybe that becomes another problem? [Not applicable.]
    
* Talk about why the problems that we list are relevant for personalized FL and not for FL in general? [Optional]

* Under the related works section, also talk about the FL evaluation framework? [Addressed.]

* Make it explicitly clear that the metrics that we introduce can be also applied to the FL setting as well? Talk about this under the Metrics section? [Addressed.]

* In Introduction, can we briefly list down the problems and then move on to the Contributions? [Addressed.]

-------------
Others:
-------------
* Introduce QoI in the metrics section. [Addressed.]

* Show the evaluations and the interpretations in terms of the metrics applied to the QoI. [Addressed.]

* Also briefly explain DS-4? [Optional?]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
ADDRESSED:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
* On how to improve the presentation of Table 2 (related works). Maybe use a map of numbers between numbers and the names of the datasets used?

* On changing the names of the columns of Table 2? 

* On the addition of additional columns to Table 2?
    - Maybe also have a column where we check if the reported works report the number of communication rounds or not, if not mentioned then maybe that becomes another problem? [Not applicable.]
    
* Talk about why the problems that we list are relevant for personalized FL and not for FL in general? [Optional]

* Under the related works section, also talk about the FL evaluation framework? [Addressed.]

* Make it explicitly clear that the metrics that we introduce can be also applied to the FL setting as well? Talk about this under the Metrics section? [Addressed.]

* In Introduction, can we briefly list down the problems and then move on to the Contributions? [Addressed.]

* Introduce QoI in the metrics section. [Addressed.]

* Show the evaluations and the interpretations in terms of the metrics applied to the QoI. [Addressed.]

*  Also briefly explain DS-4? [Addressed.]

* Density plots of the QoI values? [Addressed.]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
PENDING:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
EOF.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> tables/datasetNames_Mapper.tex <==
\begin{table}[!htp]
\centering
\begin{tabular}{|l|r|r}\toprule
\textbf{\#} &\textbf{Name of the Dataset} \\\midrule
\rowcolor{Gray}
1 &MNIST \\
2 &EMNIST \\
\rowcolor{Gray}
3 &CIFAR-10 \\
4 &CIFAR-100 \\
\rowcolor{Gray}
5 &FLICKR-AES \\
6 &Synthetic \\
\rowcolor{Gray}
7 &Shakespeare \\
8 &FEMNIST \\
\rowcolor{Gray}
9 &Sentiment 140 \\
10 &
\begin{tabular}[c]{@{}c@{}}
    Industrial \\ Recommendation Task \\
\end{tabular} \\
\rowcolor{Gray}
11 &Google Glass (GLEAM) \\
12 &
\begin{tabular}[c]{@{}c@{}}
    Human Activity \\ Recognition (HAR) \\
\end{tabular} \\
\rowcolor{Gray}
13 &Vehicle Sensor \\
14 & 
\begin{tabular}[c]{@{}c@{}}
    Mobile Assessment for \\ Prediction of Suicide (MAPS) 
\end{tabular} \\
\rowcolor{Gray}
15 &FMNIST \\
\bottomrule
\end{tabular}
\caption{Mapping between the placeholder numbers and the dataset names.}
\label{tab:datasetNames_Mapper}
\end{table}

==> tables/fairness_CIFAR10.tex <==
\begin{table*}[!htp]\centering
\setlength\tabcolsep{8pt}
\resizebox{\textwidth}{!}
{
\begin{tabular}{l|rrr|rrr|rrr|rrr|rrr|r}\toprule
\textbf{} &\multicolumn{3}{c|}{\textbf{\sysKD}} &\multicolumn{3}{c|}{\textbf{\sysGD}} &\multicolumn{3}{c|}{\textbf{FedPer}} &\multicolumn{3}{c|}{\textbf{pFedMe}} &\multicolumn{3}{c|}{\textbf{PerFed}} \\\cmidrule{2-16}
\textbf{Metrics} &\textbf{DS-1} &\textbf{DS-2} &\textbf{DS-3} &\textbf{DS-1} &\textbf{DS-2} &\textbf{DS-3} &\textbf{DS-1} &\textbf{DS-2} &\textbf{DS-3} &\textbf{DS-1} &\textbf{DS-2} &\textbf{DS-3} &\textbf{DS-1} &\textbf{DS-2} &\textbf{DS-3} \\\midrule
Average variance &21.553 &2.518 &46.66 &21.523 &2.238 &49.479 &28.595 &4.195 &56.603 &40.035 &1.806 &76.746 &23.553 &1.89 &80.53 \\
Cosine similarity &0.998395 &0.999645 &0.996572 &0.998381 &0.999669 &0.996308 &0.997667 &0.99931 &0.995519 &0.995816 &0.999742 &0.993762 &0.997381 &0.999715 &0.993412 \\
Entropy &3.31693 &3.321414 &3.316935 &3.31961 &3.321451 &3.316552 &3.318587 &3.320928 &3.315408 &3.315929 &3.321556 &3.312865 &3.318151 &3.321515 &3.312279 \\
Jain's index &0.99679 &0.99929 &0.993157 &0.99676 &0.999338 &0.99263 &0.99534 &0.998621 &0.991059 &0.99164 &0.999484 &0.987563 &0.99476 &0.99943 &0.986867 \\
\bottomrule
\end{tabular}
}
\caption{Fairness metrics applied to different personalization algorithms on CIFAR-10.}
\label{tab:fairness_CIFAR10}
\end{table*}
